WACA: Wearable-Assisted Continuous Authentication

One-time login process in conventional authentication systems does not guarantee that the identified user is the actual user throughout the session. However, it is necessary to re-verify the user identity periodically throughout a login session without reducing the user convenience. Continuous authentication can address this issue. However, existing methods are either not reliable or not usable. In this paper, we introduce a usable and reliable method called Wearable Assisted Continuous Authentication (WACA). WACA relies on the sensor based keystroke dynamics, where the authentication data is acquired through the built in sensors of a wearable (e.g., smartwatch) while the user is typing. We implemented the WACA framework and evaluated its performance on real devices with real users. The empirical evaluation of WACA reveals that WACA is feasible and its error rate is as low as 1 percent with 30 seconds of processing time and 2 3% for 20 seconds. The computational overhead is minimal. Furthermore, we tested WACA against different attack scenarios. WACA is capable of identifying insider threats with very high accuracy (99.2%) and also robust against powerful adversaries such as imitation and statistical attackers.

==> identification2.tex <==


\section{Identification Results}

\begin{table*}
    %\centering
        \caption{Scenario 1: Same text is used for both training and testing, "Multilayer Perceptron" \label{iden_same2}}
    \quad
    \quad
     \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|ccccccc|}
    \multicolumn{8}{c}{\textbf{Accuracy (\%)}} \\  \hline
    sample size  &       &       &       &       &       &       &  \\  \hline
    1500 & 77.8  & 93.7  & 97.2  & 98.4  & 99.2  & 92.9  & 100 \\
   1000 & 62.8  & 87.6  & 93.8  & 95.3  & 97.1  & 98.4  & 99.2 \\
    500 & 37.5  & 63.7  & 75.9  & 83.1  & 89.6  & 96.4  & 97 \\
    250 & 28.5  & 43    & 53.1  & 61.8  & 62.1  & 92.2  & 93.5 \\  \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & 33\%  & 66\% \\ \hline
    
    \end{tabular}
    \end{tabular}
    }
    \resizebox{\columnwidth}{!}{%
    %\quad
    \begin{tabular}{cc}
    \begin{tabular}{|c|ccccccc|}
  
    \multicolumn{8}{c}{\textbf{Weighted FPR}} \\ \hline
    Sample size &       &       &       &       &       &       &  \\ \hline
    1500  & 0.013 & 0.003 & 0.002 & 0.001 & 0     & 0.004 & 0 \\
    1000  & 0.02  & 0.007 & 0.003 & 0.003 & 0.002 & 0.001 & 0.001 \\
    500   & 0.033 & 0.019 & 0.013 & 0.009 & 0.006 & 0.002 & 0.002 \\
    250   & 0.037 & 0.029 & 0.024 & 0.019 & 0.019 & 0.004 & 0.004 \\ \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & 33\%  & 66\% \\
      \hline
    \end{tabular}
    \end{tabular}  }
\end{table*}

\begin{table*}
   % \centering
   \quad \quad
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|ccccccc|}
\multicolumn{8}{c}{\textbf{Time taken to build model (seconds)}} \\ \hline
    Sample size &       &       &       &       &       &       &  \\ \hline
    1500  & 0.99  & 2.02  & 3     & 3.99  & 4.94  & 12.67 & 12.7 \\
    1000  & 1     & 1.99  & 2.98  & 3.95  & 4.94  & 19.3  & 19.39 \\
    500   & 0.98  & 2.02  & 3.01  & 3.98  & 4.95  & 39.61 & 38.72 \\
    250   & 1     & 1.95  & 2.93  & 3.92  & 4.95  & 77.17 & 78.71 \\ \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & 33\%  & 66\% \\
     \hline
    
    \end{tabular}
    \end{tabular}
  }
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|ccccccc|}
      \multicolumn{8}{c}{\textbf{Weighted ROC Area}} \\   \hline
    Sample size &       &       &       &       &       &       &  \\   \hline
    1500  & 0.983 & 0.999 & 1     & 1     & 1     & 0.997 & 1 \\
    1000  & 0.966 & 0.994 & 0.998 & 0.999 & 1     & 1     & 1 \\
    500   & 0.883 & 0.952 & 0.981 & 0.989 & 0.991 & 0.998 & 0.999 \\
    250   & 0.805 & 0.892 & 0.925 & 0.946 & 0.954 & 0.994 & 0.995 \\   \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & 33\%  & 66\% \\
      \hline
    
    \end{tabular}
    \end{tabular} }
\end{table*}

\begin{table*}
    \centering
    
    \caption{Scenario  2:  Trained  with  exp2 (fixed-text)  and tested using exp1 (free-text), ”Multilayer Perceptron” \label{iden_diff2}}
    
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|cccccc|}
    
   \multicolumn{7}{c}{\textbf{Accuracy (\%)}} \\ \hline
    Sample size &       &       &       &       &       &  \\ \hline
    1500  & 55.8  & 80.1  & 88.7  & 89.8  & 91.8  & 93.4 \\
    1000  & 51.7  & 82.7  & 83.2  & 86.1  & 86.8  & 92 \\
    500   & 29.9  & 51.3  & 66.7  & 73.8  & 76.5  & 89.9 \\
    250   & 22.1  & 33.6  & 41.9  & 49.8  & 54.1  & 84.5 \\ \hline
      Training Set    & 1     & 2     & 3     & 4     & 5     & full \\ \hline
    
    \end{tabular}
    \end{tabular} }
    \quad
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|cccccc|}
  
    \multicolumn{7}{c}{\textbf{Weighted FPR}} \\  \hline
    Sample size &       &       &       &       &       &  \\  \hline
    1500  & 0.026 & 0.011 & 0.007 & 0.006 & 0.005 & 0.004 \\
    1000  & 0.028 & 0.01  & 0.009 & 0.008 & 0.08  & 0.005 \\
    500   & 0.04  & 0.028 & 0.019 & 0.015 & 0.013 & 0.006 \\
    250   & 0.042 & 0.036 & 0.03  & 0.027 & 0.024 & 0.009 \\  \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & full \\  \hline
    \end{tabular}
    \end{tabular}}
\end{table*}

\begin{table*}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|cccccc|}

    \multicolumn{7}{c}{\textbf{Time taken to build model (seconds)}} \\ \hline
    Sample size &       &       &       &       &       &  \\ \hline
    1500  & 1     & 1.97  & 2.97  & 4.01  & 4.99  & 12.46 \\
    1000  & 1     & 1.99  & 2.95  & 4.04  & 4.93  & 19.3 \\
    500   & 0.99  & 2     & 2.98  & 3.98  & 4.98  & 38.94 \\
    250   & 0.99  & 1.96  & 3.02  & 3.96  & 4.96  & 77.46 \\ \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & full \\ \hline
    
    \end{tabular}
    \end{tabular}}
    \quad
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc}
    \begin{tabular}{|c|cccccc|}
  
    \multicolumn{7}{c}{\textbf{Weighted ROC Area}} \\ \hline
    Sample size &       &       &       &       &       &  \\ \hline
    1500  & 0.965 & 0.992 & 0.998 & 0.998 & 0.999 & 0.998 \\
    1000  & 0.929 & 0.99  & 0.994 & 0.994 & 0.997 & 0.997 \\
    500   & 0.826 & 0.928 & 0.968 & 0.979 & 0.984 & 0.997 \\
    250   & 0.77  & 0.857 & 0.894 & 0.92  & 0.93  & 0.989 \\ \hline
    Training Set & 1     & 2     & 3     & 4     & 5     & full \\  \hline
    
    \end{tabular}
    \end{tabular}}
\end{table*}

\par In order to test the performance of some well-known ML algorithms on our data, we use Scenario 2 and plot results on Figure~\ref{ml_comp_training} and \ref{ml_comp_samples}.




Figure~\ref{ml_comp_training} compares the different ML algorithms for different size o training sets when the sample size is 1500. All of algorithms increasing with the increasing number of training samples as expected. When we look at different algorithms, while NaiveBayes is almost linearly increasing, the others start to converge to a value around 90\%-92\%.
On the other hand, Figure~\ref{ml_comp_samples} compares different ML algorithms for different different sample sizes while number of training samples is 5. It is clear that in Figure~\ref{ml_comp_samples}, all algorithms perform similar and are increasing with the sample size.

\begin{figure}[h]
    \centering
          \includegraphics[width=.5\textwidth,trim= 0cm 9cm 0cm 9cm]{compare_mls}
          \caption{Comparing different ML algorithms for different size of the training sets, for constant sample size=1500  \label{ml_comp_training}}
\end{figure}

\begin{figure}[h]
    \centering
          \includegraphics[width=.5\textwidth,trim= 0cm 9cm 0cm 8cm]{compare_mls2}
          \caption{Comparing different ML algorithms for different sample sizes for constant 5 training samples  \label{ml_comp_samples}}
\end{figure}
